Efficient Output Kernel Learning for Multiple Tasks

The paradigm of multi-task learning is that one can achieve better generalization by learning tasks jointly and thus exploiting the similarity between the tasks rather than learning them independently of each other. While previously the relationship between tasks had to be user-defined in the form of an output kernel, recent approaches jointly learn the tasks and the output kernel. As the output kernel is a positive semidefinite matrix, the resulting optimization problems are not scalable in the number of tasks as an eigendecomposition is required in each step. \mbox{Using} the theory of positive semidefinite kernels we show in this paper that for a certain class of regularizers on the output kernel, the constraint of being positive semidefinite can be dropped as it is automatically satisfied for the relaxed problem. This leads to an unconstrained dual problem which can be solved efficiently. Experiments on several multi-task and multi-class data sets illustrate the efficacy of our approach in terms of computational efficiency as well as generalization performance.

==> figures/figure-eta-cnn.tex <==
\begin{figure}[t]\small\centering
% \vspace*{0.75em}
\includegraphics[width=0.5\columnwidth]{Gain_in_time_vs_Eta.pdf}%
\caption{%
Factor by which the proposed optimization approach outperforms OKL over the hyper-parameter range on various data sets with maximum number of tasks.  We outperform OKL on average by a factor of $8.4$ on MIT Indoor67 and by $5.2$ on SUN397 data sets. 
As mentioned in Section~\ref{sec:specialDual}, the number of hyper-parameters in~\eqref{eq:final-dual} is reduced to one. The expression of $\eta$ is given by $\eta=\frac{\lambda C^3}{(4k-2)} \Big(\frac{2k-1}{2k\lambda}\Big)^{2k}$ for general $p$-norm, where $p=\frac{2k}{2k-1}$. 
}\label{fig:eta-cnn}
\end{figure}


==> figures/figure-scaling-cnn.tex <==
\begin{figure}[t]\small\centering
\caption{%
Scaling experiment on SUN397 with Places205 CNN kernel and $m=5$.
%The optimization procedure proposed in Algorithm~\ref{alg:sdca}
%scales roughly linearly with the number of tasks.
Our approach \oursquared is seven times faster that OKL when number of tasks is highest and its efficiency is comparable with the single task learning approach (STL-SDCA). 
%Moreover, for $T=50\ldots200$ the runtime of \oursquared is roughly comparable to the STL baseline, which makes the method particularly attractive.
}\label{fig:scaling-cnn}
\vspace*{0.75em}
\includegraphics[width=0.4\columnwidth]{Plot_Time_vs_NumTask_june4.pdf}%
\end{figure}


==> figures/figure-scaling-fv.tex <==
\begin{figure}[t]\small\centering
\vspace*{0.75em}
\includegraphics[width=0.4\columnwidth]{scaling-fv.pdf}%
\caption{%
Scaling experiment on SUN397 with a Fisher Vector kernel and $m=5$.
%The optimization procedure proposed in Algorithm~\ref{alg:sdca}
%scales roughly linearly with the number of tasks.
Our approach \oursquared is about an order of magnitude faster than OKL in this setting
and scales well with the number of tasks.
%Moreover, for $T=50\ldots200$ the runtime of \oursquared is roughly comparable to the STL baseline, which makes the method particularly attractive.
}\label{fig:scaling-fv}
\end{figure}


==> figures/figure-suboptimality.tex <==
\begin{figure}[t]\small\centering
\caption{%
Plot comparing the rate of convergence between the proposed \oursquared and OKL~\citep{Dinuzzo11} on SUN397 with a Fisher Vector kernel. Note that \oursquared achieves lower objectives an order of magnitude faster than OKL. 
}\label{fig:suboptimality-fv}
\vspace*{0.75em}
\includegraphics[width=0.7\columnwidth]{suboptimality-fv.pdf}%
\end{figure}


==> figures/figure-theta-matrix.tex <==
\begin{figure}[t]\small\centering
\caption{%
Qualitative evaluation of the proposed method \oursquared on SUN397
in the best setting (CNN features, $m=50$).
}\label{fig:theta-matrix}
\vspace*{0.75em}
\includegraphics[width=0.1\columnwidth]{theta-2.pdf}%
\end{figure}


==> figures/table-indoor67.tex <==
\begin{table}[ht]\centering\small
\caption{Performance on the MIT Indoor67 dataset.
}\label{tbl:indoor67}
\vspace*{0.75em}
\begin{tabular}{l|c}\toprule
Method & Accuracy \\
\midrule
\midrule
%\cite{zheng2012learning} & 47.2 \\
%\cite{juneja2013blocks} & 63.10 \\
%\cite{bu2013superpixel} & 48.3 \\
%\cite{doersch2013mid} & 66.87 \\
%\cite{sun2013learning} & 51.4 \\
\citep{razavian2014cnn} & $58.4$ \\
\citep{zhou2014learning} & $68.24$ \\
\citep{gong2014multi} & $68.88$ \\
%\cite{razavian2014cnn}+aug & 69.0 \\
\citep{koskela2014convolutional} & $70.1$ \\
\midrule
STL & $71.5$ \\
\ourmethodHinge $(q=4)$ & $71.6$ \\
\ourmethodSquare $(q=4)$ & $\mathbf{73.4}$ \\
\bottomrule
\end{tabular}
\end{table}


==> figures/table-mnist-usps.tex <==
\begin{table*}[ht]\centering
{\tiny
\caption{Performance of various methods on regression and classification datasets. The first row of each dataset reports the mean generalization performance over ten random train-test splits. The second row reports the standard deviation.}\label{table:mnistusps}
\begin{tabular}{llccccc}\toprule
Method & Dataset & Ntrain=5 & Ntrain=10 & Ntrain=20 & Ntrain=50 & Ntrain=100\\
\midrule
\midrule
Kang et.al \cite{kang2011learning} & & & & & & 84.8 (0.3) \\
MTRL \cite{??} & & 64.8 (1.5) & 73.7 (0.6) & 78.8 (0.1) & 83.9 (0.5) & 85.6 (0.4) \\
STL-SDCA & MNIST \cite{kang2011learning} & 65.6 (0.7) & 73.6 (0.8) & 79.8 (1.0) & 83.1 (0.6) & 85.7 (0.4) \\
MTL-SDCA & & 66.2 (0.7) & 74.0 (1.0) & 79.7 (0.9) & 83.4 (0.6) & 86.0 (0.2) \\
Our (squared, cv-pow-10) & & 65.9 (1.0) & 72.0 (1.0) & 77.4 (0.3) & 81.2 (0.5) & 82.3 (0.6) \\
Our (squared, cv-pow-2) & & 66.5 (0.9) & 72.5 (1.0) & 77.6 (0.4) & 81.2 (0.5) & 82.2 (0.6) \\
Our (hinge, cv-pow-10) & & 65.3 (1.3) & 73.2 (0.9) & 78.5 (0.2) & 83.3 (0.2) & 86.2 (0.3) \\
Our (hinge, cv-pow-2) & & 65.2 (1.3) & 73.4 (0.6) & 78.6 (0.2) & 83.7 (0.2) & 86.1 (0.3) \\
\midrule
Kang et.al \cite{kang2011learning} & & & & & & 91.6 (0.3) \\
MTRL \cite{??} & & 68.4 (1.7) & 78.6 (0.8) & 85.0 (0.3) & 90.3 (0.6) & 92.4 (0.2) \\
STL-SDCA & USPS \cite{kang2011learning} & 69.4 (0.6) & 76.3 (1.1) & 83.7 (0.2) & 88.5 (0.5) & 90.8 (0.3) \\
MTL-SDCA & & 71.4 (0.7) & 77.2 (0.5) & 84.6 (0.4) & 90.0 (0.5) & 90.6 (0.2) \\
Our (squared, cv-pow-10) & & 69.2 (1.6) & 76.0 (0.9) & 81.8 (0.6) & 86.3 (0.5) & 87.6 (0.3) \\
Our (squared, cv-pow-2) & & 69.2 (1.6) & 76.2 (1.3) & 81.4 (0.6) & 86.0 (0.4) & 87.3 (0.4) \\
Our (hinge, cv-pow-10) & & 70.4 (1.5) & 78.7 (0.9) & 84.9 (0.6) & 90.0 (0.5) & 92.3 (0.2) \\
Our (hinge, cv-pow-2) & & 70.6 (2.0) & 78.4 (0.9) & 84.4 (0.4) & 90.1 (0.6) & 92.4 (0.3) \\
\bottomrule
\end{tabular}
}
\end{table*}


==> figures/table-mnist-usps_b.tex <==
\begin{table}[t]\centering\scriptsize
\caption{Mean accuracy and standard deviation reported on various multi-class data sets. %over five train-test splits. % on handwritten recognition data sets. 
%The proposed \ourmethodHingeq{8} achieves the best accuracy in both data sets. 
}\label{table:mnistusps}
% \vspace*{0.75em}
\renewcommand{\tabcolsep}{0.3em}
\begin{tabular}{l|c|ccc|cc|cc}\toprule
\multirow{2}{*}{\textbf{Data set}} &
\multirow{2}{*}{\textbf{STL}} &
\multirow{2}{*}{\textbf{MTL-SDCA}} &
\multirow{2}{*}{\textbf{GMTL}} &
\multirow{2}{*}{\textbf{MTRL}} &
\multicolumn{2}{c|}{\textbf{\ourmethodHinge}}&
\multicolumn{2}{c}{\textbf{\ourmethodSquare}}\\%&
% \multirow{2}{*}{\textbf{\ourmethodKL}}\\
 & & & & & $p=2$ & $p=8/7$ & $p=2$ & $p=8/7$\\
\midrule
\midrule
MNIST & $84.1\pm0.3$ & $86.0\pm0.2$ & $84.8\pm0.3$ & $85.6\pm0.4$ & $86.1\pm0.4$ & $\mathbf{86.2\pm0.4}$ & $82.3\pm0.6$ & $82.4\pm0.3$ \\
USPS  & $90.5\pm0.3$ & $90.6\pm0.2$ & $91.6\pm0.3$ & $92.4\pm0.2$ & $92.4\pm0.2$ & $\mathbf{92.6\pm0.1}$ & $87.2\pm0.4$ & $87.5\pm0.3$ \\
SUN397 ($m=5$) & $43.7\pm1.2$& $41.2\pm1.3$ & - & - & $41.5\pm1.1$ & $41.6\pm1.2$ & $\mathbf{44.1\pm1.3}$ & $44.0\pm1.2$ \\
SUN397 ($m=50$) & $\mathbf{58.6\pm0.1}$& $54.8\pm0.3$ & - & - & $55.1\pm0.2$ & $55.1\pm0.3$ & $\mathbf{58.6\pm0.1}$ & $\mathbf{58.6\pm0.2}$\\
% STL & $84.1\pm0.3$ & $90.5\pm0.3$\\
% GMTL & $84.8\pm0.3$ & $91.6\pm0.3$ \\
% MTRL & $85.6\pm0.4$ & $\mathbf{92.4\pm0.2}$ \\
% MTL-SDCA & $86.0\pm0.2$ & $90.6\pm0.2$ \\
% \oursquared & $82.2\pm0.6$ & $87.3\pm0.4$ \\
% \ourhinge & $\mathbf{86.1\pm0.3}$ & $\mathbf{92.4\pm0.3}$ \\
\bottomrule
\end{tabular}
\end{table}

% \begin{table}[ht]\centering\small
% \caption{Performance on handwritten digit recognition datasets.
% }\label{table:mnistusps}
% \vspace*{0.75em}
% \begin{tabular}{l|c|c}\toprule
%  & MNIST & USPS\\
% \midrule
% \midrule
% STL & $84.1\pm0.3$ & $90.5\pm0.3$\\
% GMTL & $84.8\pm0.3$ & $91.6\pm0.3$ \\
% MTRL & $85.6\pm0.4$ & $\mathbf{92.4\pm0.2}$ \\
% MTL-SDCA & $86.0\pm0.2$ & $90.6\pm0.2$ \\
% \oursquared & $82.2\pm0.6$ & $87.3\pm0.4$ \\
% \ourhinge & $\mathbf{86.1\pm0.3}$ & $\mathbf{92.4\pm0.3}$ \\
% \bottomrule
% \end{tabular}
% \end{table}


==> figures/table-multi-task-old.tex <==
\begin{table*}\centering\scriptsize
\caption{Performance of various methods on regression and classification datasets. The first row of each dataset reports the mean generalization performance over ten random train-test splits. The second row reports the standard deviation.
Our proposed method, \ourmethod, is overall the best method on 4 out of 6 datasets.
}\label{table:resultPerf}
\vspace*{1em}
\begin{tabular}{ll|llllll|lll}\toprule
\multirow{2}{*}{\textbf{Dataset}} &
\multirow{2}{*}{\textbf{STL}} &
\multirow{2}{*}{\textbf{MTL}} &
\multirow{2}{*}{\textbf{CMTL}} &
\multirow{2}{*}{\textbf{DMTL}} &
\multirow{2}{*}{\textbf{MTFL}} &
\multirow{2}{*}{\textbf{GMTL}} &
\multirow{2}{*}{\textbf{MTRL}} &
\multicolumn{3}{c}{\textbf{\ourmethod}}\\
 & & & & & & & & $q=2$ & $q=4$ & $q=8$ \\
\midrule
\midrule
\multicolumn{11}{l}{Regression Datasets: Explained Variance (\%)} \\\\

% {SARCOS} & $40.47\pm7.56$ & $34.50\pm10.19$ & $33.02\pm13.42$ & $40.59\pm10.24$ & $\mathbf{49.86\pm6.34}$ & $45.77\pm10.63$ & $9.50\pm15.84$
% \\
{Sarcos} & $40.47$ & $34.50$ & $33.02$ & $40.59$ & $49.86$ & $45.77$ & $41.63$ & $46.71$ & $\mathbf{50.33}$ & $48.35$
\\
 & $(\pm7.56)$ & $(\pm10.19)$ & $(\pm13.42)$ & $(\pm10.24)$ & $(\pm6.34)$ & $(\pm10.63)$ & $(\pm7.12)$ & $(\pm6.89)$ & $(\pm5.81)$ & $(\pm5.81)$
\\& & & & & & & & & \\
% {PARKINSON} & $2.84\pm7.51$ & $4.94\pm19.95$ & $2.74\pm3.62$ & $-12.25\pm7.41$ & $\mathbf{16.79\pm10.81}$ & $33.61\pm9.36$ & $0.71\pm23.79$
% \\
{Parkinson} & $2.84$ & $4.94$ & $2.74$ & $-12.25$ & $16.79$ & $\mathbf{33.61}$ & $12.02$ & $27.01$ & $27.01$ & $27.01$
\\
 & $(\pm7.51)$ & $(\pm19.95)$ & $(\pm3.62)$ & $(\pm7.41)$ & $(\pm10.81)$ & $(\pm9.36)$ & $(\pm6.76)$ & $(\pm4.43)$ & $(\pm4.43)$ & $(\pm4.43)$
\\
\midrule
\multicolumn{11}{l}{Classification Datasets: AUC (\%)} \\\\
% {YALE} & $93.36\pm2.33$ & $96.35\pm1.64$ & $95.20\pm2.12$ & $92.44\pm2.81$ & $\mathbf{96.98\pm1.55}$ & $91.91\pm3.19$ & $89.04\pm7.62$
% \\
{Yale} & $93.36$ & $96.35$ & $95.20$ & $92.44$ & $96.98$ & $91.91$ & $96.08$ & $\mathbf{97.02}$ & $96.95$ & $96.83$
\\
 & $(\pm2.33)$ & $(\pm1.64)$ & $(\pm2.12)$ & $(\pm2.81)$ & $(\pm1.55)$ & $(\pm3.19)$ & $(\pm2.07)$ & $(\pm1.19)$ & $(\pm1.40)$ & $(\pm1.43)$
\\& & & & & & & & & \\

% {LANDMINE} & $74.60\pm1.55$ & $76.42\pm0.78$ & $75.86\pm0.66$ & $65.86\pm2.63$ & $\mathbf{76.44\pm0.92}$ & $76.72\pm1.23$ & $69.77\pm7.36$
% \\
{Landmine} & $74.60$ & $76.42$ & $75.86$ & $65.86$ & $76.44$ & $76.72$ & $76.08$ & $\mathbf{76.83}$ & $76.68$ & $76.38$ 
\\

 & $(\pm1.55)$ & $(\pm0.78)$ & $(\pm0.66)$ & $(\pm2.63)$ & $(\pm0.92)$ & $(\pm1.23)$ & $(\pm0.98)$ & $(\pm0.79)$ & $(\pm0.96)$ & $(\pm0.86)$ 
\\& & & & & & & & & \\

% {MHC-I} & $69.25\pm2.07$ & $72.28\pm1.94$ & $\mathbf{72.56\pm1.36}$ & $58.39\pm5.46$ & $71.68\pm2.20$ & $72.54\pm2.71$ & $66.20\pm6.84$
% \\
{MHC-I} & $69.25$ & $72.28$ & $\mathbf{72.56}$ & $58.39$ & $71.68$ & $72.54$ & $71.51$ & $71.69$ & $70.78$ & $70.68$ 
\\
  & $(\pm2.07)$ & $(\pm1.94)$ & $(\pm1.36)$ & $(\pm5.46)$ & $(\pm2.20)$ & $(\pm2.71)$ & $(\pm1.74)$ & $(\pm1.92)$ & $(\pm2.14)$ & $(\pm1.85)$
\\& & & & & & & & & \\

% {LETTER} & $\mathbf{61.24\pm0.82}$ & $61.02\pm1.56$ & $60.52\pm1.09$ & $59.34\pm1.39$ & $60.45\pm1.75$ & $61.22\pm0.85$ & $59.68\pm2.88$
% \\
{Letter} & $61.24$ & $61.02$ & $60.52$ & $59.34$ & $60.45$ & $61.22$ & $60.25$ & $61.42$ & $\mathbf{61.48}$ & $61.40$ 
\\
 & $(\pm 0.82)$ & $(\pm1.56)$ & $(\pm1.09)$ & $(\pm1.39)$ & $(\pm1.75)$ & $(\pm0.85)$ & $(\pm1.39)$ & $(\pm0.72)$ & $(\pm1.02)$ & $(\pm0.98)$ 
\\
\bottomrule
\end{tabular}
\end{table*}


==> figures/table-multi-task-with-DMTL.tex <==
\begin{table*}\centering\scriptsize
\caption{Performance of various methods on regression and classification datasets.
We report mean generalization performance and the standard deviation
over ten random train-test splits.
Our proposed method is overall the best method in 4 out of 6 datasets.
}\label{table:resultPerf}
\vspace*{0.75em}\renewcommand{\tabcolsep}{0.3em}
\begin{tabular}{l|c|cccccc|ccc}\toprule
\multirow{2}{*}{\textbf{Dataset}} &
\multirow{2}{*}{\textbf{STL}} &
\multirow{2}{*}{\textbf{MTL}} &
\multirow{2}{*}{\textbf{CMTL}} &
\multirow{2}{*}{\textbf{DMTL}} &
\multirow{2}{*}{\textbf{MTFL}} &
\multirow{2}{*}{\textbf{GMTL}} &
\multirow{2}{*}{\textbf{MTRL}} &
\multicolumn{3}{c}{\textbf{\ourmethod}}\\
 & & & & & & & & $q=2$ & $q=4$ & $q=8$ \\
\midrule
\midrule
\multicolumn{11}{l}{Regression Datasets: Explained Variance (\%)}\vspace*{.5em} \\
{Sarcos} &
$40.5\pm7.6$ & $34.5\pm10.2$ & $33.0\pm13.4$ & $40.6\pm10.2$ & $49.9\pm6.3$ &
$45.8\pm10.6$ & $41.6\pm7.1$ & $46.7\pm6.9$ & $\mathbf{50.3\pm5.8}$ & $48.4\pm5.8$ \\
{Parkinson} &
$2.8\pm7.5$ & $4.9\pm20.0$ & $2.7\pm3.6$ & $-12.3\pm7.4$ & $16.8\pm10.8$ &
$\mathbf{33.6\pm9.4}$ & $12.0\pm6.8$ & $27.0\pm4.4$ & $27.0\pm4.4$ & $27.0\pm4.4$ \\
\midrule
\multicolumn{11}{l}{Classification Datasets: AUC (\%)}\vspace*{.5em} \\
{Yale} &
$93.4\pm2.3$ & $96.4\pm1.6$ & $95.2\pm2.1$ & $92.4\pm2.8$ & $\mathbf{97.0\pm1.6}$ &
$91.9\pm3.2$ & $96.1\pm2.1$ & $\mathbf{97.0\pm1.2}$ & $\mathbf{97.0\pm1.4}$ & $96.8\pm1.4$ \\
{Landmine} &
$74.6\pm1.6$ & $76.4\pm0.8$ & $75.9\pm0.7$ & $65.9\pm2.6$ & $76.4\pm1.0$ &
$76.7\pm1.2$ & $76.1\pm1.0$ & $\mathbf{76.8\pm0.8}$ & $76.7\pm1.0$ & $76.4\pm0.9$ \\
{MHC-I} &
$69.3\pm2.1$ & $72.3\pm1.9$ & $\mathbf{72.6\pm1.4}$ & $58.4\pm5.5$ & $71.7\pm2.2$ &
$72.5\pm2.7$ & $71.5\pm1.7$ & $71.7\pm1.9$ & $70.8\pm2.1$ & $70.7\pm1.9$ \\
{Letter} &
$61.2\pm0.8$ & $61.0\pm1.6$ & $60.5\pm1.1$ & $59.3\pm1.4$ & $60.5\pm1.8$ &
$61.2\pm0.9$ & $60.3\pm1.4$ & $61.4\pm0.7$ & $\mathbf{61.5\pm1.0}$ & $61.4\pm1.0$ \\
\bottomrule
\end{tabular}
\end{table*}


==> figures/table-speedup.tex <==
\begin{table}[t]\centering%\scriptsize
\caption{Average speed up factor of \ourmethodSquare over OKL on various data sets. % on handwritten recognition data sets. 
%The proposed \ourmethodHingeq{8} achieves the best accuracy in both data sets. 
}\label{table:speedup}
% \vspace*{0.75em}
% \renewcommand{\tabcolsep}{0.3em}
\begin{tabular}{cccc}\toprule
SUN397 & MIT Indoor67 & MNIST & USPS\\
\midrule
\midrule
5.2 & 8.4 & 24.1 & 24.2\\
% STL & $84.1\pm0.3$ & $90.5\pm0.3$\\
% GMTL & $84.8\pm0.3$ & $91.6\pm0.3$ \\
% MTRL & $85.6\pm0.4$ & $\mathbf{92.4\pm0.2}$ \\
% MTL-SDCA & $86.0\pm0.2$ & $90.6\pm0.2$ \\
% \oursquared & $82.2\pm0.6$ & $87.3\pm0.4$ \\
% \ourhinge & $\mathbf{86.1\pm0.3}$ & $\mathbf{92.4\pm0.3}$ \\
\bottomrule
\end{tabular}
\end{table}


==> figures/table-sun397-old.tex <==
\begin{table*}[ht]\centering
{\scriptsize
\caption{Performance on the SUN397 benchmark.
We report mean accuracy and the standard deviation over ten available train-test splits.
Our method, \ourmethodSquare achieves the current state of the art results
for all $m=5,\ldots,50$ with the Places205 CNN features.
}\label{table:sun397cvpr14}
\vspace*{0.75em}
\begin{tabular}{lc|cccc}\toprule
Method & Features & $m=5$ & $m=10$ & $m=20$ & $m=50$ \\
\midrule
\midrule
%\citep{xiao2010sun} & 12 combined & $14.5$ & $20.9$ & $28.1$ & $38.0$ \\
%\citep{su2012improving} & Context+Semantic &  &  &  & $35.6\pm0.4$ \\
%\citep{donahue2013decaf} & DeCAF$_6$ &  &  &  & $40.9\pm0.3$ \\
\citep{gong2014multi} & \multirow{2}{*}{ImageNet CNN} &  &  &  & $51.98$ \\
\citep{koskela2014convolutional} & &  &  &  & $54.65\pm0.2$ \\
\citep{zhou2014learning} & Places205 CNN &  &  &  & $54.32\pm0.1$ \\
\midrule
% \citep{sanchez2013image} & \multirow{9}{*}{\parbox{7em}{\centering Fisher Vector (SIFT+Color)}}
% & $21.1\pm0.3$ & $29.1\pm0.3$ & $37.4\pm0.3$ & $47.2\pm0.2$ \\
% STL-SDCA & & $22.1\pm0.6$ & $30.5\pm0.6$ & $38.8\pm0.3$ & $48.4\pm0.2$ \\
% MTL-SDCA & & $22.4\pm0.5$ & $31.0\pm0.7$ & $39.5\pm0.3$ & $49.5\pm0.3$ \\
% \ourmethodHinge $(q=2)$ & & $22.1\pm1.0$ & $31.0\pm0.9$ & $39.1\pm0.4$ & $48.8\pm0.3$ \\
% \ourmethodHinge $(q=4)$ & & $22.0\pm1.1$ & $30.9\pm0.9$ & $38.9\pm0.5$ & $48.7\pm0.3$\\
% \ourmethodHinge $(q=8)$ & & $22.2\pm1.0$ & $30.9\pm0.9$ & $38.9\pm0.5$ & $48.7\pm0.3$\\
% \ourmethodSquare $(q=2$) & & $21.6\pm1.1$ & $29.1\pm0.8$ & $36.4\pm0.5$ & $44.6\pm0.2$ \\
% \ourmethodSquare $(q=4)$ & & $21.6\pm1.1$ & $29.2\pm0.8$ & $36.4\pm0.5$ & $44.9\pm0.2$\\
% \ourmethodSquare $(q=8)$ & & $21.6\pm1.0$ & $29.2\pm0.7$ & $36.4\pm0.4$ & $44.7\pm0.2$\\
% \midrule
STL-SDCA & \multirow{8}{*}{Places205 CNN} &
$40.5\pm0.9$ & $46.6\pm0.5$ & $51.2\pm0.5$ & $55.0\pm0.4$ \\
MTL-SDCA & & $41.2\pm1.3$ & $46.7\pm0.5$ & $51.1\pm0.5$ & $54.8\pm0.3$ \\
\ourmethodHinge $(q=2)$ & & $41.4\pm1.1$ & $46.9\pm0.4$ & $51.0\pm0.6$ & $55.1\pm0.2$ \\
\ourmethodHinge $(q=4$) & & $41.6\pm1.3$ & $47.3\pm0.4$  & $51.5\pm0.6$ & $55.4\pm0.3$ \\
\ourmethodHinge $(q=8)$ & & $41.7\pm1.2$ & $47.0\pm0.4$ & $51.3\pm0.6$ & $56.5\pm0.2$ \\
\ourmethodSquare $(q=2)$ & & $42.4\pm1.3$ & $47.8\pm0.5$ & $53.5\pm0.4$ & $\mathbf{58.6\pm0.1}$ \\
\ourmethodSquare $(q=4)$ & & $43.9\pm1.2$ & $49.5\pm0.5$ & $54.2\pm0.3$ & $\mathbf{58.6\pm0.1}$ \\
\ourmethodSquare $(q=8)$ & & $\mathbf{44.1\pm1.2}$ & $\mathbf{49.7\pm0.6}$ & $\mathbf{54.3\pm0.3}$ & $58.5\pm0.1$ \\
\bottomrule
\end{tabular}
}
\end{table*}


==> figures/table-sun397.tex <==
\begin{table*}[t]\centering
{\scriptsize
\caption{Performance on the SUN397. We report mean accuracy and the standard deviation over ten train-test splits.
Our methods, \ourmethodSquare and \ourmethodKL achieves significantly better results. %for all $m=5,\ldots,50$. 
}\label{table:sun397cvpr14}
% \vspace*{0.75em}
\renewcommand{\tabcolsep}{0.5em}
\begin{tabular}{l|c|c|ccc|ccc|c}\toprule
\multirow{2}{*}{\textbf{$m$}} &
\multirow{2}{*}{\textbf{STL}} &
\multirow{2}{*}{\textbf{MTL-SDCA}} &
\multicolumn{3}{c|}{\textbf{\ourmethodHinge}}&
\multicolumn{3}{c|}{\textbf{\ourmethodSquare}}&
\multirow{2}{*}{\textbf{\ourmethodKL}}\\
 & & & $p=2$ & $p=4/3$ & $p=8/7$ & $p=2$ & $p=4/3$ & $p=8/7$ & \\
\midrule
\midrule
\ \ $5$ & $40.5\pm0.9$& $41.2\pm1.3$& $41.5\pm1.1$& $41.6\pm1.3$ & $41.6\pm1.2$ & $\mathbf{44.1\pm1.3}$& $\mathbf{44.1\pm1.1}$& $44.0\pm1.2$ & $\mathbf{44.1\pm1.3}$\\
   $10$ & $46.6\pm0.5$& $46.7\pm0.5$& $46.9\pm0.4$& $47.2\pm0.4$ & $47.1\pm0.5$ & $49.5\pm0.5$         & $\mathbf{49.7\pm0.4}$& $49.6\pm0.5$ & $49.6\pm0.5$\\
   $20$ & $51.2\pm0.5$& $51.1\pm0.5$& $51.0\pm0.6$& $51.8\pm0.6$ & $51.4\pm0.6$ & $54.2\pm0.4$         & $\mathbf{54.3\pm0.3}$& $54.2\pm0.3$ & $54.2\pm0.4$\\
   $50$ & $55.0\pm0.4$& $54.8\pm0.3$& $55.1\pm0.2$& $55.6\pm0.3$ & $55.1\pm0.3$ & $\mathbf{58.6\pm0.1}$& $58.5\pm0.1$         & $\mathbf{58.6\pm0.2}$ & $58.4\pm0.1$  \\
%\citep{xiao2010sun} & 12 combined & $14.5$ & $20.9$ & $28.1$ & $38.0$ \\
%\citep{su2012improving} & Context+Semantic &  &  &  & $35.6\pm0.4$ \\
%\citep{donahue2013decaf} & DeCAF$_6$ &  &  &  & $40.9\pm0.3$ \\
% \citep{gong2014multi} & \multirow{2}{*}{ImageNet CNN} &  &  &  & $51.98$ \\
% \citep{koskela2014convolutional} & &  &  &  & $54.65\pm0.2$ \\
% \citep{zhou2014learning} & Places205 CNN &  &  &  & $54.32\pm0.1$ \\
% \midrule
% \citep{sanchez2013image} & \multirow{9}{*}{\parbox{7em}{\centering Fisher Vector (SIFT+Color)}}
% & $21.1\pm0.3$ & $29.1\pm0.3$ & $37.4\pm0.3$ & $47.2\pm0.2$ \\
% STL-SDCA & & $22.1\pm0.6$ & $30.5\pm0.6$ & $38.8\pm0.3$ & $48.4\pm0.2$ \\
% MTL-SDCA & & $22.4\pm0.5$ & $31.0\pm0.7$ & $39.5\pm0.3$ & $49.5\pm0.3$ \\
% \ourmethodHinge $(q=2)$ & & $22.1\pm1.0$ & $31.0\pm0.9$ & $39.1\pm0.4$ & $48.8\pm0.3$ \\
% \ourmethodHinge $(q=4)$ & & $22.0\pm1.1$ & $30.9\pm0.9$ & $38.9\pm0.5$ & $48.7\pm0.3$\\
% \ourmethodHinge $(q=8)$ & & $22.2\pm1.0$ & $30.9\pm0.9$ & $38.9\pm0.5$ & $48.7\pm0.3$\\
% \ourmethodSquare $(q=2$) & & $21.6\pm1.1$ & $29.1\pm0.8$ & $36.4\pm0.5$ & $44.6\pm0.2$ \\
% \ourmethodSquare $(q=4)$ & & $21.6\pm1.1$ & $29.2\pm0.8$ & $36.4\pm0.5$ & $44.9\pm0.2$\\
% \ourmethodSquare $(q=8)$ & & $21.6\pm1.0$ & $29.2\pm0.7$ & $36.4\pm0.4$ & $44.7\pm0.2$\\
% \midrule
% STL-SDCA & \multirow{8}{*}{Places205 CNN} &
% 			    $40.5\pm0.9$ & $46.6\pm0.5$ & $51.2\pm0.5$ & $55.0\pm0.4$ \\
% 		MTL-SDCA & & $41.2\pm1.3$ & $46.7\pm0.5$ & $51.1\pm0.5$ & $54.8\pm0.3$ \\
% \ourmethodHinge $(q=2)$ & & $41.4\pm1.1$ & $46.9\pm0.4$ & $51.0\pm0.6$ & $55.1\pm0.2$ \\
% \ourmethodHinge $(q=4$) & & $41.6\pm1.3$ & $47.3\pm0.4$  & $51.5\pm0.6$ & $55.4\pm0.3$ \\
% \ourmethodHinge $(q=8)$ & & $41.7\pm1.2$ & $47.0\pm0.4$ & $51.3\pm0.6$ & $56.5\pm0.2$ \\
% \ourmethodSquare $(q=2)$ & & $42.4\pm1.3$ & $47.8\pm0.5$ & $53.5\pm0.4$ & $\mathbf{58.6\pm0.1}$ \\
% \ourmethodSquare $(q=4)$ & & $43.9\pm1.2$ & $49.5\pm0.5$ & $54.2\pm0.3$ & $\mathbf{58.6\pm0.1}$ \\
% \ourmethodSquare $(q=8)$ & & $\mathbf{44.1\pm1.2}$ & $\mathbf{49.7\pm0.6}$ & $\mathbf{54.3\pm0.3}$ & $58.5\pm0.1$ \\
\bottomrule
\end{tabular}
}
\end{table*}


==> figures/table-sun397_withoutKL.tex <==
\begin{table*}[t]\centering
{\scriptsize
\caption{Performance on the SUN397. We report mean accuracy and the standard deviation over ten available train-test splits.
Our method, \ourmethodSquare achieves significantly better results. %for all $m=5,\ldots,50$.
}\label{table:sun397cvpr14}
% \vspace*{0.75em}
\begin{tabular}{l|c|c|ccc|ccc}\toprule
\multirow{2}{*}{\textbf{$m$}} &
\multirow{2}{*}{\textbf{STL}} &
\multirow{2}{*}{\textbf{MTL-SDCA}} &
\multicolumn{3}{c|}{\textbf{\ourmethodHinge}}&
\multicolumn{3}{c}{\textbf{\ourmethodSquare}}\\
 & & & $p=2$ & $p=4/3$ & $p=8/7$ & $p=2$ & $p=4/3$ & $p=8/7$\\
\midrule
\midrule
\ \ $5$ & $40.5\pm0.9$& $41.2\pm1.3$& $41.5\pm1.1$& $41.6\pm1.3$ & $41.6\pm1.2$ & $\mathbf{44.1\pm1.3}$& $\mathbf{44.1\pm1.1}$& $44.0\pm1.2$ \\
   $10$ & $46.6\pm0.5$& $46.7\pm0.5$& $46.9\pm0.4$& $47.2\pm0.4$ & $47.1\pm0.5$ & $49.5\pm0.5$         & $\mathbf{49.7\pm0.4}$& $49.6\pm0.5$\\
   $20$ & $51.2\pm0.5$& $51.1\pm0.5$& $51.0\pm0.6$& $51.8\pm0.6$ & $51.4\pm0.6$ & $54.2\pm0.4$         & $\mathbf{54.3\pm0.3}$& $54.2\pm0.3$ \\
   $50$ & $55.0\pm0.4$& $54.8\pm0.3$& $55.1\pm0.2$& $55.6\pm0.3$ & $55.1\pm0.3$ & $\mathbf{58.6\pm0.1}$& $58.5\pm0.1$         & $\mathbf{58.6\pm0.2}$ \\
%\citep{xiao2010sun} & 12 combined & $14.5$ & $20.9$ & $28.1$ & $38.0$ \\
%\citep{su2012improving} & Context+Semantic &  &  &  & $35.6\pm0.4$ \\
%\citep{donahue2013decaf} & DeCAF$_6$ &  &  &  & $40.9\pm0.3$ \\
% \citep{gong2014multi} & \multirow{2}{*}{ImageNet CNN} &  &  &  & $51.98$ \\
% \citep{koskela2014convolutional} & &  &  &  & $54.65\pm0.2$ \\
% \citep{zhou2014learning} & Places205 CNN &  &  &  & $54.32\pm0.1$ \\
% \midrule
% \citep{sanchez2013image} & \multirow{9}{*}{\parbox{7em}{\centering Fisher Vector (SIFT+Color)}}
% & $21.1\pm0.3$ & $29.1\pm0.3$ & $37.4\pm0.3$ & $47.2\pm0.2$ \\
% STL-SDCA & & $22.1\pm0.6$ & $30.5\pm0.6$ & $38.8\pm0.3$ & $48.4\pm0.2$ \\
% MTL-SDCA & & $22.4\pm0.5$ & $31.0\pm0.7$ & $39.5\pm0.3$ & $49.5\pm0.3$ \\
% \ourmethodHinge $(q=2)$ & & $22.1\pm1.0$ & $31.0\pm0.9$ & $39.1\pm0.4$ & $48.8\pm0.3$ \\
% \ourmethodHinge $(q=4)$ & & $22.0\pm1.1$ & $30.9\pm0.9$ & $38.9\pm0.5$ & $48.7\pm0.3$\\
% \ourmethodHinge $(q=8)$ & & $22.2\pm1.0$ & $30.9\pm0.9$ & $38.9\pm0.5$ & $48.7\pm0.3$\\
% \ourmethodSquare $(q=2$) & & $21.6\pm1.1$ & $29.1\pm0.8$ & $36.4\pm0.5$ & $44.6\pm0.2$ \\
% \ourmethodSquare $(q=4)$ & & $21.6\pm1.1$ & $29.2\pm0.8$ & $36.4\pm0.5$ & $44.9\pm0.2$\\
% \ourmethodSquare $(q=8)$ & & $21.6\pm1.0$ & $29.2\pm0.7$ & $36.4\pm0.4$ & $44.7\pm0.2$\\
% \midrule
% STL-SDCA & \multirow{8}{*}{Places205 CNN} &
% 			    $40.5\pm0.9$ & $46.6\pm0.5$ & $51.2\pm0.5$ & $55.0\pm0.4$ \\
% 		MTL-SDCA & & $41.2\pm1.3$ & $46.7\pm0.5$ & $51.1\pm0.5$ & $54.8\pm0.3$ \\
% \ourmethodHinge $(q=2)$ & & $41.4\pm1.1$ & $46.9\pm0.4$ & $51.0\pm0.6$ & $55.1\pm0.2$ \\
% \ourmethodHinge $(q=4$) & & $41.6\pm1.3$ & $47.3\pm0.4$  & $51.5\pm0.6$ & $55.4\pm0.3$ \\
% \ourmethodHinge $(q=8)$ & & $41.7\pm1.2$ & $47.0\pm0.4$ & $51.3\pm0.6$ & $56.5\pm0.2$ \\
% \ourmethodSquare $(q=2)$ & & $42.4\pm1.3$ & $47.8\pm0.5$ & $53.5\pm0.4$ & $\mathbf{58.6\pm0.1}$ \\
% \ourmethodSquare $(q=4)$ & & $43.9\pm1.2$ & $49.5\pm0.5$ & $54.2\pm0.3$ & $\mathbf{58.6\pm0.1}$ \\
% \ourmethodSquare $(q=8)$ & & $\mathbf{44.1\pm1.2}$ & $\mathbf{49.7\pm0.6}$ & $\mathbf{54.3\pm0.3}$ & $58.5\pm0.1$ \\
\bottomrule
\end{tabular}
}
\end{table*}

